EDM: An Ultra-Low Latency Ethernet Fabric for Memory Disaggregation

Achieving low remote memory access latency remains the primary challenge in realizing memory disaggregation over Ethernet within the datacenters. We present EDM that attempts to overcome this challenge using two key ideas. First, while existing network protocols for remote memory access over the Ethernet, such as TCP/IP and RDMA, are implemented on top of the MAC layer, EDM takes a radical approach by implementing the entire network protocol stack for remote memory access within the Physical layer (PHY) of the Ethernet. This overcomes fundamental latency and bandwidth overheads imposed by the MAC layer, especially for small memory messages. Second, EDM implements a centralized, fast, in-network scheduler for memory traffic within the PHY of the Ethernet switch. Inspired by the classic Parallel Iterative Matching (PIM) algorithm, the scheduler dynamically reserves bandwidth between compute and memory nodes by creating virtual circuits in the PHY, thus eliminating queuing delay and layer 2 packet processing delay at the switch for memory traffic, while maintaining high bandwidth utilization. Our FPGA testbed demonstrates that EDM's network fabric incurs a latency of only $\sim$300 ns for remote memory access in an unloaded network, which is an order of magnitude lower than state-of-the-art Ethernet-based solutions such as RoCEv2 and comparable to emerging PCIe-based solutions such as CXL. Larger-scale network simulations indicate that even at high network loads, EDM's average latency remains within 1.3$\times$ its unloaded latency.

==> cc.tex <==
% New definitions
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
\algtext*{EndSwitch}%
\algtext*{EndCase}%

\section{CC Note}
\label{sec:cc}

In general, the send-host initiates a transaction by sending a notification block before being granted from ToR. Each port grants one flow until it finishes. The notification and grant block includes port numbers, request type (RREQ, WREQ) and flow size. 

In the specific case of Read operation, since the RREQ is small, EDM does not apply notification but directly forwards it instead. Upon ToR receiving the first block of RREQ, it already knows that the receiver of this RREQ will soon initiate a RRESP, of which the receiver is the RREQ requester. Thus the ToR automatically creates a grant, if available, for the destination host.

Moreover, in order to reach full throughput when network is loaded with incast, i.e., pipelining forwarding plane, EDM will release egress port and give grant in \textbf{one BDP} advance so that the next flow seamlessly takes over without further awaits.

Note that the end host could also experience buffer overflow, we require each receiver host to send a pause signal to ToR if their receiving buffer grows above a threshold. The ToR then stops granting any new flows destined to the paused host until it sends a resume signal.

Formalized cc protocol is shwon in Algorithm.\ref{algo:cc sender},\ref{algo:cc ToR},\ref{algo:cc recv}:
\begin{algorithm}
\caption{Sender}
   \begin{algorithmic}[h]
\State Check Send Buffer:
\Switch{$blk\_type$}
\Case{$RREQ$}
\State Send Blk;Seq\_num++;
\EndCase
\Case{$RRESP$}
\If{Granted}
\State Send blk; Seq\_num++;
\EndIf
\EndCase
\Case{$WREQ$}
\If{Granted}
\State Send blk; Seq\_num++;
\Else 
    \If{Un-notified}
        \State Send Notification;
    \EndIf
\EndIf
\EndCase
\EndSwitch
\end{algorithmic} 
\label{algo:cc sender}
\end{algorithm}

\begin{algorithm}
\caption{ToR}
    \begin{algorithmic}[h]
    \Switch{$blk\_type$}
        \Case{$RREQ\_Header$}
            \State Create Notification $ntf$;
            \State $NotificationQueue \gets ntf$;
            \State Forward blk to blk->Dst;
        \EndCase
        \Case{$Notification$}
            \State Create Notification $ntf$;
            \State $NotificationQueue \gets ntf$;
        \EndCase
        \Case{$PAUSE$}
            \State Lock port[blk->Src];
        \EndCase
        \Case{$RESUME$}
            \State Release port[blk->Src];
        \EndCase
        \Case{$Default$}
            \State Forward blk to blk->Dst;
            \If{Remaining $FlowSize \leq BDP$}
                \State Release port[blk->Dst];
            \EndIf
        \EndCase
        \EndSwitch
    \For{ntf in NotificationQueue}
        \If{port[ntf->Dst] is free}
            \State Create Grant grt;
            \State Forward grt to ntf->Dst;
            \State Lock port[ntf->Dst];
        \EndIf
    \EndFor
    \end{algorithmic}
\label{algo:cc ToR}
\end{algorithm}

\begin{algorithm}
\caption{Receiver}
    \begin{algorithmic}
    \Switch{$blk\_type$}
        \Case{$Grant$}
            \State Mark flow[grt->flowID] granted;
        \EndCase
        \Case{$Default$}
            \State Mark received;
        \EndCase
    \EndSwitch
    \If{$Buffer\geq THRES$}
        \State $SendBuffer \gets PAUSE$
    \EndIf
    \If{ Paused and $Buffer < THRES$}
        \State $SendBuffer \gets RESUME$
    \EndIf
    \end{algorithmic}
\label{algo:cc recv}
\end{algorithm}



